Dynamic Learning of Correlation Potentials for a Time-Dependent Kohn-Sham System

We develop methods to learn the correlation potential for a time-dependent Kohn-Sham (TDKS) system in one spatial dimension. We start from a low-dimensional two-electron system for which we can numerically solve the time-dependent Schr\"odinger equation; this yields electron densities suitable for training models of the correlation potential. We frame the learning problem as one of optimizing a least-squares objective subject to the constraint that the dynamics obey the TDKS equation. Applying adjoints, we develop efficient methods to compute gradients and thereby learn models of the correlation potential. Our results show that it is possible to learn values of the correlation potential such that the resulting electron densities match ground truth densities. We also show how to learn correlation potential functionals with memory, demonstrating one such model that yields reasonable results for trajectories outside the training set.

==> snipped.tex <==
With (\ref{eqn:adjsys}), the final expression (\ref{eqn:deltaL}) for $\delta \mathscr{L}$ reduces to
\begin{equation}
\label{eqn:deltaLfinal}
\delta \mathscr{L} = \Re \left\{ \left( 2 \left[ (|\bphi_0|^2 - \tilde{\bn}_0) \circ \bphi_0 \right]^\dagger + \blambda^\dagger_{1} \nabla_{\bphi} \bF_{\Delta t} (\bphi_0,\bv_{C}(t_0) ) \right) \delta \bphi_{0} \right\}
\end{equation}

complex variables is
\begin{multline*}
\mathscr{L}(\bPhi, \bLambda, \bv^{C}) = \frac{1}{2} \sum_{k=0}^{K} \sum_{j=-J}^{J} ( 2 \phi(x_j, t_k)^\ast \phi(x_j, t_k) - \tilde{n}(x_j, t_k) )^2 \\
- \Re \sum_{k=0}^{K-1} \blambda_{k+1}^\dagger \left( \bphi_{k+1}  - \bF_{\Delta t}(\bphi_k, \bv^{C}_k) \right).
\end{multline*}
To prepare to take real variations, we rewrite this Lagrangian as a function of

% 

% \begin{itemize}
% \item Neural network model of $v^C$ as a functional of current and previous $\phi$.   Train with $p=-1.0$ and $p=-1.8$, predict on the rest.  See Figure \ref{fig:vCphimemory}.
% We have trained using (black) reference electron densities computed from the 2D Schr\"odinger equation with initial momenta equal to $p=-1.0$ and $p=-1.8$.  The (blue) test set electron densities correspond to $p=-1.2$, $p=-1.4$, $p=-1.5$, and $p=-1.6$
% \item Neural network model of $v^C$ as a functional of current and previous $n$.  Train with $p=-1.0$ and $p=-1.8$, predict on the rest.  See Figure \ref{fig:vCnvecmemory}.
% \end{itemize}


% In these methods, we do not need ground-truth values of $v^{C}$.  To learn $v^C$, we minimize the mismatch between observed and predicted electron densities, with the dynamics of $\Phi$ constrained by the discretized TDKS equation. 

